Large Language Models are Fixated by Red Herrings: Exploring Creative Problem Solving and Einstellung Effect using the Only Connect Wall Dataset

The quest for human imitative AI has been an enduring topic in AI research since its inception. The technical evolution and emerging capabilities of the latest cohort of large language models (LLMs) have reinvigorated the subject beyond academia to the cultural zeitgeist. While recent NLP evaluation benchmark tasks test some aspects of human-imitative behaviour (e.g., BIG-bench's 'human-like behavior' tasks), few, if not none, examine creative problem solving abilities. Creative problem solving in humans is a well-studied topic in cognitive neuroscience with standardized tests that predominantly use the ability to associate (heterogeneous) connections among clue words as a metric for creativity. Exposure to misleading stimuli - distractors dubbed red herrings - impede human performance in such tasks via the fixation effect and Einstellung paradigm. In cognitive neuroscience studies, such fixations are experimentally induced by pre-exposing participants to orthographically similar incorrect words to subsequent word-fragments or clues. The popular British quiz show Only Connect's Connecting Wall segment essentially mimics Mednick's Remote Associates Test (RAT) formulation with built-in, deliberate red herrings, which makes it an ideal proxy dataset to explore and study fixation effect and Einstellung paradigm from cognitive neuroscience in LLMs. In this paper we present the novel Only Connect Wall (OCW) dataset and report results from our evaluation of selected pre-trained language models and LLMs on creative problem solving tasks like grouping clue words by heterogeneous connections, and identifying correct open knowledge domain connections in respective groups. We synthetically generate two additional datasets: OCW-Randomized, OCW-WordNet to further analyze our red-herrings hypothesis in language models. The code and link to the dataset are available at https://github.com/TaatiTeam/OCW.

==> sections/10_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

With rapid advances in LLMs, standardized benchmarks and tasks for systemic evaluation of NLP models are saturated. In this work, we curated a dataset and challenging tasks in which SOTA models, including GPT-4, still underperform humans by a large margin. The dataset provides a new benchmark to evaluate reasoning abilities and general intelligence.
%
% Future work includes augmenting the dataset with connecting walls from newer seasons of the quiz show as well as with fan-generated walls.\footnote{\url{https://puzzgrid.com/} contains over 4200 user-generated connecting walls and solutions at 5 different difficulty levels.}


% \footnote{As of March 2023, Season 18 is ending and Season 19 is commissioned.} 


==> sections/45_checklists.tex <==
% See \href{Neurips2023}{https://neurips.cc/Conferences/2023/PaperInformation/StyleFiles}
% guidelines. Checklist is submitted via openreview portal, should not be included in pdf.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count toward the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \autoref{sec:limitations}}
  \item Did you discuss any potential negative social impacts of your work?
    \answerYes{{See \autoref{sec:Datasheet}}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results~(either in the supplemental material or as a URL)?
    \answerYes{See \url{https://github.com/TaatiTeam/OCW}}
  \item Did you specify all the training details~(e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \autoref{subsec_tasks}.}
        \item Did you report error bars~(e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See standard deviation in the tables (e.g. \autoref{tab:task1-results-static})}
        \item Did you include the total amount of computing and the type of resources used~(e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \autoref{sec:Datasheet}}
\end{enumerate}


\item If you are using existing assets~(e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Our dataset is released under a MIT license, see \autoref{sec:Datasheet}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See \url{https://github.com/TaatiTeam/OCW}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All data was curated from the quiz show Only Connect, which is publicly available; no information from participants on the show, besides anonymized and aggregated performance statistics, was collected. The statistics refer to the scores of the CWs (solved/partially solved/unsolved) rather than the players}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{To the best of our knowledge, the curated data does not contain any PII or offensive content}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board~(IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/52_app_neurips_datasheet.tex <==
\section{Datasheet}\label{sec:Datasheet}
The following section provides answers to questions listed in datasheets for datasets.

% \todo{Appendix with more dataset specific info is needed.}

% \todo{Next to a scientific paper, authors should also submit supplementary materials such as detail on how the data was collected and organized, what kind of information it contains, how it should be used ethically and responsibly, as well as how it will be made available and maintained."}
% \footnote{\url{https://en.wikipedia.org/wiki/Lord\%27s}} 
 % Clusters of connected words in each wall emerge when embeddings are projected to 2-dimensions using t-SNE. Colors and shapes correspond to true clusters, and grey convex regions correspond to predicted clusters. Legend shows the ground truth connection for each group.
 
% \todo{maybe also say something about future work to safeguard against data contamination?}

\newcommand{\sectioncolor}{violet}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{mdframed}
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    MOTIVATION
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    For what purpose was the dataset created?
    }
    Was there a specific task in mind? Was there
    a specific gap that needed to be filled? Please provide a description.
    } \\
    
    %%%
    The OCW dataset is created to be an analogical proxy for the Remote Associates Test~(RAT)~\cite{mednick1968remote} from cognitive neuroscience in evaluating LLMs for human-imitative \textit{creative problem-solving}. The presented clues have heterogeneous connections with open-domain knowledge retrieval and contain red herrings or misleading stimuli by design. The two tasks entails \textit{grouping} sixteen~(16) jumbled up clue words into associated groups, and naming the right \textit{connection} for each group. To the best of our knowledge, there are no existing tasks for evaluating LLMs for human-like creative problem solving in existing, and concurrent benchmarks including the BIG-Bench, HELM, Global-Bench. Thus, this dataset and tasks are valuable additions for overall LLM evaluation and measuring progress towards human-imitative AI.
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Who created this dataset (e.g., which team, research group) and on behalf
    of which entity (e.g., company, institution, organization)?
    }
    } \\
    %%%
    The dataset has been collectively curated by the authors of this paper. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What support was needed to make this dataset?
    }
    (e.g.who funded the creation of the dataset? If there is an associated
    grant, provide the name of the grantor and the grant name and number, or if
    it was supported by a company or government agency, give those details.)
    } \\
    %%%
    This work was supported by Natural Sciences and Engineering Research Council of Canada (NSERC). \\
    %%% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    COMPOSITION
}}
\end{mdframed}
    \textcolor{\sectioncolor}{\textbf{
    What do the instances that comprise the dataset represent (e.g., documents,
    photos, people, countries)?
    }
    Are there multiple types of instances (e.g., movies, users, and ratings;
    people and interactions between them; nodes and edges)? Please provide a
    description.
    } \\
    %%%
    % OCW contains clues with their corresponding connections. 
    Each instance contains a connecting wall puzzle and its solution from the popular quiz show Only Connect.\\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    How many instances are there in total (of each type, if appropriate)?
    }
    } \\
    %%%
    618 wall puzzles (instances of the dataset), for a total of 2,472 groups, and 9,888 clues.\\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain all possible instances or is it a sample (not
    necessarily random) of instances from a larger set?
    }
    } \\
    %%%
    The dataset has been curated from the first fifteen seasons of the "Only Connect" show, which accounts for approximately 81\% of the total seasons. The latest season, Season 18, was concluded in March 2023.
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What data does each instance consist of?
    }
    “Raw” data (e.g., unprocessed text or images) or features? In either case,
    please provide a description.
    } \\
    %%%
    Each instance contains a connecting wall puzzle and its clues and solution. All instances are in English and provided as text strings in JSON format.\\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is there a label or target associated with each instance?
    }
    If so, please provide a description.
    } \\
    %%%
    Yes. The labels for Task 1 are the solved walls, and for Task 2 the ground-truth connections. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is any information missing from individual instances?
    }
    If so, please provide a description, explaining why this information is
    missing (e.g., because it was unavailable). This does not include
    intentionally removed information, but might include, e.g., redacted text.
    } \\
    %%%
    N/A \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Are relationships between individual instances made explicit (e.g., users’
    movie ratings, social network links)?
    }
    If so, please describe how these relationships are made explicit.
    } \\
    %%%
    Each wall is given a unique ID. Clues and solutions associated with each wall belong to the same JSON object as that wall.\\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Are there recommended data splits (e.g., training, development/validation,
    testing)?
    }
    If so, please provide a description of these splits, explaining the
    rationale behind them.
    } \\
    %%%
    We randomly split the dataset into the training/dev/test set according to a proportion of 1:1:8. The primary goal of our dataset is to evaluate the zero- and few-shot creative problem-solving abilities of Large Language Models; as such, we elect to set the size of the test set to be much greater than train or validation sets. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Are there any errors, sources of noise, or redundancies in the dataset?
    }
    If so, please provide a description.
    } \\
    %%%
    The dataset has undergone a thorough review and is subjected to both automated and manual checks as part of a strict quality control protocol. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is the dataset self-contained, or does it link to or otherwise rely on
    external resources (e.g., websites, tweets, other datasets)?
    }
    } \\
    %%%
    The dataset is self-contained. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain data that might be considered confidential (e.g.,
    data that is protected by legal privilege or by doctor-patient
    confidentiality, data that includes the content of individuals’ non-public
    communications)?
    }
    If so, please provide a description.
    } \\
    %%%
    N/A. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain data that, if viewed directly, might be offensive,
    insulting, threatening, or might otherwise cause anxiety?
    }
    If so, please describe why.
    } \\
    %%%
    N/A. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset relate to people?
    }
    If not, you may skip the remaining questions in this section.
    } \\
    %%%
    The dataset does not have individual-specific information. \\
    %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Does the dataset identify any subpopulations (e.g., by age, gender)?
    % }
    % If so, please describe how these subpopulations are identified and
    % provide a description of their respective distributions within the dataset.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Is it possible to identify individuals (i.e., one or more natural persons),
    % either directly or indirectly (i.e., in combination with other data) from
    % the dataset?
    % }
    % If so, please describe how.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Does the dataset contain data that might be considered sensitive in any way
    % (e.g., data that reveals racial or ethnic origins, sexual orientations,
    % religious beliefs, political opinions or union memberships, or locations;
    % financial or health data; biometric or genetic data; forms of government
    % identification, such as social security numbers; criminal history)?
    % }
    % If so, please provide a description.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Any other comments?
    % }} \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    COLLECTION
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    How was the data associated with each instance acquired?
    }
    Was the data directly observable (e.g., raw text, movie ratings),
    reported by subjects (e.g., survey responses), or indirectly
    inferred/derived from other data (e.g., part-of-speech tags, model-based
    guesses for age or language)? If data was reported by subjects or
    indirectly inferred/derived from other data, was the data
    validated/verified? If so, please describe how.
    } \\
    %%%
    The wall puzzles were scraped from the fan website ocdb.cc as well as manually watching the episodes. Human performance results were manually curated from the episodes. all data verified through manual watching of episodes. \\
    %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Over what timeframe was the data collected?
    % }
    % Does this timeframe match the creation timeframe of the data associated
    % with the instances (e.g., recent crawl of old news articles)? If not,
    % please describe the timeframe in which the data associated with the
    % instances was created. Finally, list when the dataset was first published.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What mechanisms or procedures were used to collect the data (e.g., hardware
    apparatus or sensor, manual human curation, software program, software
    API)?
    }
    How were these mechanisms or procedures validated?
    } \\
    %%%
    We utilized python's BeautifulSoup library to scrape only connect fan websites. all episodes were watched manually for human performance collection, and the same procedure validated the data collection.\\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What was the resource cost of collecting the data?
    }
    (e.g. what were the required computational resources, and the associated
    financial costs
    } \\
    %%%
    Experiments were run using NVIDIA GeForce RTX 2080 Ti GPU system. \\
    %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % If the dataset is a sample from a larger set, what was the sampling
    % strategy (e.g., deterministic, probabilistic with specific sampling
    % probabilities)?
    % }
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Who was involved in the data collection process (e.g., students,
    crowdworkers, contractors) and how were they compensated (e.g., how much
    were crowdworkers paid)?
    }
    } \\
    %%%
    The authors of this paper. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Were any ethical review processes conducted (e.g., by an institutional
    review board)?
    }
    If so, please provide a description of these review processes, including
    the outcomes, as well as a link or other access point to any supporting
    documentation.
    } \\
    %%%
    N/A. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset relate to people?
    }
    If not, you may skip the remainder of the questions in this section.
    } \\
    %%%
    The dataset does not have individual-specific information. \\
    %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Did you collect the data from the individuals in question directly, or
    % obtain it via third parties or other sources (e.g., websites)?
    % }
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Were the individuals in question notified about the data collection?
    % }
    % If so, please describe (or show with screenshots or other information) how
    % notice was provided, and provide a link or other access point to, or
    % otherwise reproduce, the exact language of the notification itself.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Did the individuals in question consent to the collection and use of their
    % data?
    % }
    % If so, please describe (or show with screenshots or other information) how
    % consent was requested and provided, and provide a link or other access
    % point to, or otherwise reproduce, the exact language to which the
    % individuals consented.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % If consent was obtained, were the consenting individuals provided with a
    % mechanism to revoke their consent in the future or for certain uses?
    % }
    %  If so, please provide a description, as well as a link or other access
    %  point to the mechanism (if appropriate)
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Has an analysis of the potential impact of the dataset and its use on data
    % subjects (e.g., a data protection impact analysis)been conducted?
    % }
    % If so, please provide a description of this analysis, including the
    % outcomes, as well as a link or other access point to any supporting
    % documentation.
    % } \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%% 
    
    % \textcolor{\sectioncolor}{\textbf{
    % Any other comments?
    % }} \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    PREPROCESSING / CLEANING / LABELING
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Was any preprocessing/cleaning/labeling of the data
    done(e.g.,discretization or bucketing, tokenization, part-of-speech
    tagging, SIFT feature extraction, removal of instances, processing of
    missing values)?
    }
    If so, please provide a description. If not, you may skip the remainder of
    the questions in this section.
    } \\
    %%%
    N/A. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Was the “raw” data saved in addition to the preprocessed/cleaned/labeled
    data (e.g., to support unanticipated future uses)?
    }
    If so, please provide a link or other access point to the “raw” data.
    } \\
    %%%
    N/A. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is the software used to preprocess/clean/label the instances available?
    }
    If so, please provide a link or other access point.
    } \\
    %%%
    N/A. \\
    %%%

    % \textcolor{\sectioncolor}{\textbf{
    % Any other comments?
    % }} \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    USES
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Has the dataset been used for any tasks already?
    }
    If so, please provide a description.
    } \\
    %%%
    No. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is there a repository that links to any or all papers or systems that use the dataset?
    }
    If so, please provide a link or other access point.
    } \\
    %%%
    No. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    What (other) tasks could the dataset be used for?
    }
    } \\
    %%%
     Evaluation of Large Language Models for creative problem-solving as well as Artificial General Intelligence tasks. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is there anything about the composition of the dataset or the way it was
    collected and preprocessed/cleaned/labeled that might impact future uses?
    }
    For example, is there anything that a future user might need to know to
    avoid uses that could result in unfair treatment of individuals or groups
    (e.g., stereotyping, quality of service issues) or other undesirable harms
    (e.g., financial harms, legal risks) If so, please provide a description.
    Is there anything a future user could do to mitigate these undesirable
    harms?
    } \\
    %%%
    N/A. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Are there tasks for which the dataset should not be used?
    }
    If so, please provide a description.
    } \\
    %%%
    We caution regarding unethical reuse of the dataset, specifically for the purpose of training future reasoning engines for unethical use cases. \\
    %%%

    % \textcolor{\sectioncolor}{\textbf{
    % Any other comments?
    % }} \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    DISTRIBUTION
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Will the dataset be distributed to third parties outside of the entity
    (e.g., company, institution, organization) on behalf of which the dataset
    was created?
    }
    If so, please provide a description.
    } \\
    %%%
    No. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    How will the dataset will be distributed (e.g., tarball on website, API,
    GitHub)?
    }
    Does the dataset have a digital object identifier (DOI)?
    } \\
    %%%
    The code and link to the dataset is available at \url{https://github.com/TaatiTeam/OCW} \\
    % as well as at \url{}
    % The dataset can be directly downloaded at \url{https://www.cs.toronto.edu/~taati/OCW/OCW.tar.gz} \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    When will the dataset be distributed?
    }
    } \\
    %%%
    Now.  \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Will the dataset be distributed under a copyright or other intellectual
    property (IP) license, and/or under applicable terms of use (ToU)?
    }
    If so, please describe this license and/or ToU, and provide a link or other
    access point to, or otherwise reproduce, any relevant licensing terms or
    ToU, as well as any fees associated with these restrictions.
    } \\
    %%%
    The dataset is released under MIT License. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Have any third parties imposed IP-based or other restrictions on the data
    associated with the instances?
    }
    If so, please describe these restrictions, and provide a link or other
    access point to, or otherwise reproduce, any relevant licensing terms, as
    well as any fees associated with these restrictions.
    } \\
    %%%
    No. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Do any export controls or other regulatory restrictions apply to the
    dataset or to individual instances?
    }
    If so, please describe these restrictions, and provide a link or other
    access point to, or otherwise reproduce, any supporting documentation.
    } \\
    %%%
    No. \\
    %%%

    % \textcolor{\sectioncolor}{\textbf{
    % Any other comments?
    % }} \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    MAINTENANCE
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Who is supporting/hosting/maintaining the dataset?
    }
    } \\
    %%%
    The dataset is hosted on University of Toronto Computer Science Department servers and will be maintained by the authors of this paper. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    How can the owner/curator/manager of the dataset be contacted (e.g., email
    address)?
    }
    } \\
    %%%
    The maintainers can be contacted via email: saeid.alavi@mail.utoronto.ca, raeidsaqur@cs.toronto.edu, john.giorgi@mail.utoronto.ca, mozhgans@stanford.edu, babak.taati@uhn.ca. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is there an erratum?
    }
    If so, please provide a link or other access point.
    } \\
    %%%
    No. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Will the dataset be updated (e.g., to correct labeling errors, add new
    instances, delete instances)?
    }
    If so, please describe how often, by whom, and how updates will be
    communicated to users (e.g., mailing list, GitHub)?
    } \\
    %%%
    The authors plan to continue updating the dataset, including but not limited to scaling the dataset to include more seasons, providing new test/dev sets, and organizing shared tasks with the dataset. The updates will be yearly and communicated to users through public shared tasks. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    If the dataset relates to people, are there applicable limits on the
    retention of the data associated with the instances (e.g., were individuals
    in question told that their data would be retained for a fixed period of
    time and then deleted)?
    }
    If so, please describe these limits and explain how they will be enforced.
    } \\
    %%%
    N/A. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Will older versions of the dataset continue to be
    supported/hosted/maintained?
    }
    If so, please describe how. If not, please describe how its obsolescence
    will be communicated to users.
    } \\
    %%%
    Yes, the authors are committed to maintaining and updating the older versions of the dataset. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    If others want to extend/augment/build on/contribute to the dataset, is
    there a mechanism for them to do so?
    }
    If so, please provide a description. Will these contributions be
    validated/verified? If so, please describe how. If not, why not? Is there a
    process for communicating/distributing these contributions to other users?
    If so, please provide a description.
    } \\
    %%%
    Any potential contributors are welcome to expand the dataset to larger size through contacting the authors of the paper. \\
    %%%

    % \textcolor{\sectioncolor}{\textbf{
    % Any other comments?
    % }} \\
    % %%%
    % YOUR ANSWER HERE \\
    % %%

